dtControl2+$\varepsilon$: Trading Optimality for Explainability in MDPs via Decision Trees

Over the past decade, decision trees have been used to represent controllers (a.k.a. policies) in an explainable way, with dtControl2 as a current state-of-the-art tool. However, for systems that are large or have many corner cases, even such representations tend to be too complex and not human-comprehensible. Unfortunately, reducing the size of the decision tree is not straightforward, as missing just a single crucial case might result in an incorrect controller. We tackle this issue in the setting of Markov decision processes, extending dtControl2 by "$\varepsilon$" functionality: Given an allowed imprecision $\varepsilon \geq 0$, we construct a smaller decision tree, distilling the essence of the controller, while still guaranteeing its $\varepsilon$-optimality. This enables us to provide tunably simpler explanations, omitting a controllable amount of detail. Our tool constructs decision trees that are orders of magnitude smaller than the state of the art.

==> format/macros.tex <==
\setcounter{secnumdepth}{3} 
\Crefname{subsubsubappendix}{Appendix}{Appendices}%

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}






\RequirePackage{marvosym}

\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\DeclarePairedDelimiter\abs{\lvert}{\rvert}


\newcommand{\Naturals}{\mathbb{N}}
\newcommand{\Reals}{\mathbb{R}}
\newcommand{\Distributions}{\Delta}
\newcommand{\Paths}{\mathsf{Paths}}



\DeclareMathOperator*{\argmax}{arg\, max}
\DeclareMathOperator*{\argmin}{arg\, min}
\newcommand{\post}{\mathsf{post}}
\newcommand{\eqdef}{\vcentcolon=}
\newcommand{\defeq}{=\vcentcolon}

\newcommand{\qee}{\hfill$\triangle$} %


\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\Expectation}{\mathbb{E}}

\newcommand{\MDP}{\mathcal{M}}
\newcommand{\initstate}{{\bar{s}}}
\newcommand{\states}{\mathsf{S}}
\newcommand{\actions}{\mathsf{A}}
\newcommand{\trans}{\delta}
\newcommand{\gStates}{\mathsf{G}}
\newcommand{\Reach}{\mathsf{Reach}}
\newcommand{\domain}{\mathbb{D}}
\newcommand{\reachobj}{\mathsf{P}}


\newcommand{\apath}{\rho}
\newcommand{\paths}{\mathsf{Paths}}
\newcommand{\controller}{\pi}
\newcommand{\policies}{\Pi}
\newcommand{\prob}{\mathbb{P}}
\newcommand{\opt}{\mathsf{opt}}

\newcommand{\pred}{\rho}

\spnewtheorem*{proofidea}{Proof Idea}{\itshape}{\rmfamily}




\newcommand{\val}{\mathsf{V}}


\newcommand{\orcidID}[1]{{\href{https://orcid.org/#1}{\protect\raisebox{3.25pt}{\protect\includegraphics{orcid_color}}}}}

\newcommand{\inlineheadingbf}[1]{\smallskip\noindent{\bfseries #1.}}
\newcommand{\inlineheadingbfd}[1]{\smallskip\noindent{\bfseries #1}}
\newcommand{\inlineheadingit}[1]{\smallskip\noindent{\it #1.}}


\newcommand\tool[1]{{\texttt{#1}\xspace}}
\newcommand\definetool[2]{\newcommand{#1}{\tool{#2}\xspace}}
\definetool{\dtcontrol}{dtControl\hspace*{1.3pt}2}
\definetool{\dtcontrolnonumber}{dtControl}
\definetool{\dtcontroleps}{dtControl\hspace*{2.3pt}2\hspace*{-1.pt}+$\varepsilon$}
\definetool{\storm}{Storm}
\definetool{\stormpy}{stormpy}
\definetool{\dtnest}{dtNESt}
\definetool{\dtpaynt}{dtPaynt}
\newcommand{\dte}[0]{\dtcontroleps}
\newcommand{\dtc}[0]{\dtcontrol}



\newcommand{\dtconstruct}{\texttt{DT-Construct}\xspace}
\newcommand{\earlystop}{\text{Early-Stopping}\xspace}
\newcommand{\predicates}{\texttt{Preds}\xspace}
\newcommand{\impurity}{\texttt{Impurity}\xspace}

\newcommand{\stepOne}{Model Building and Solving\xspace}
\newcommand{\stepTwo}{Dataset Construction\xspace}
\newcommand{\stepThree}{DT Learning\xspace}
\newcommand{\stepFour}{Pruning\xspace}

\newcommand{\unreach}{\texttt{Unreach}}
\newcommand{\agency}{\texttt{Agency}}
\newcommand{\dominance}{\texttt{Dominance}}
\newcommand{\singlec}{\texttt{SingleC}}
\newcommand{\allSafe}{\texttt{AllOpt}}
\newcommand{\eqval}{\texttt{EqVal}}
\newcommand{\permissive}{\texttt{GoodActions}}
\newcommand{\datasetController}{\textsf{Controller}}
\newcommand{\datasetPermissive}{\textsf{Permissive}}
\newcommand{\datasetCombined}{\textsf{Combined}}

\newcommand{\wuniform}{\texttt{Imp\_Uniform}}
\newcommand{\wcav}{\texttt{Imp\_CAV15}}
\newcommand{\wsimulation}{\texttt{Imp\_Simulation}}
\newcommand{\wagency}{\texttt{Imp\_Agency}}
\newcommand{\wmessup}{\texttt{Imp\_CoE}}

\newcommand{\decisiontree}{\mathcal{T}}
\newcommand{\uniforma}{\mathsf{Unif}}

\newcommand{\compTablePayntNestTime}{\csvcoli&\csvcoliii&\csvcolix&\csvcolvi&\csvcolxv&\csvcolxxxiii&\csvcolxxiv&\csvcolxlii&\csvcolliv&\csvcolxlviii&\csvcolxxxix&\csvcolli&\csvcolxlv}

\newcommand{\compTabletime}{\csvcoli&\csvcolxxiii&\csvcolxxiv&\csvcolxxv&\csvcolv&\csvcolvi&\csvcolvii&\csvcolxxxii&\csvcolxxxiii&\csvcolxxxiv&\csvcolxlv&\csvcolxlvi&\csvcolxlvii&\csvcolii&\csvcoliii&\csvcoliv&\csvcolxliv}
\newcommand{\compTabletreesize}{\csvcoli&\csvcolxxiii&\csvcolxxiv&\csvcolxxv&\csvcolv&\csvcolvi&\csvcolvii&\csvcolxxxii&\csvcolxxxiii&\csvcolxxxiv&\csvcolxlv&\csvcolxlvi&\csvcolxlvii&\csvcolii&\csvcoliii&\csvcoliv&\csvcolxliv&\csvcolxlix&\csvcollv&\csvcollii&\csvcollviii&\csvcollxii&\csvcollx}
\newcommand{\compStateStatisticsCombined}{\csvcoli&\csvcollxxv&\csvcolxxiii&\csvcolxxiv&\csvcolxxv&\csvcolii&\csvcoliii&\csvcoliv&\csvcolvii&\csvcolx&\csvcolxxxi}
\newcommand{\compStateStatisticsController}{\csvcoli&\csvcollxxv&\csvcollvi&\csvcollvii&\csvcollviii&\csvcolxxxv&\csvcolxxxvi&\csvcolxxxvii&\csvcolxl&\csvcolxliii&\csvcollxiv}
\newcommand{\compStateStatisticsPermissive}{\csvcoli&\csvcollxxv&\csvcolcii&\csvcolciii&\csvcolciv&\csvcollxxxi&\csvcollxxxii&\csvcollxxxiii&\csvcollxxxvi&\csvcollxxxix&\csvcolcx}

\newcommand{\compStateStatisticsAgg}{\csvcoli&\csvcolii&\csvcoliv&\csvcolv&\csvcolvi&\csvcolvii&\csvcolviii&\csvcolix&\csvcolx&\csvcolxi&\csvcolxii}
\newcommand{\compAblationDtSize}{\csvcoli&\csvcolii&\csvcoliii&\csvcoliv&\csvcolv&\csvcolvi&\csvcolvii&\csvcolviii&\csvcolix&\csvcolx&\csvcolxi}
\newcommand{\compAblationPruningSize}{\csvcoli&\csvcolii&\csvcoliii&\csvcoliv&\csvcolv&\csvcolvi&\csvcolvii&\csvcolviii&\csvcolix&\csvcolx&\csvcolxi}
\newcommand{\compBaselinePruning}{\csvcoli&\csvcolii&\csvcoliii&\csvcoliv&\csvcolv&\csvcolvi}


